Is Disaggregation possible for HPC Cognitive Simulation?

Cognitive simulation (CogSim) is an important and emerging workflow for HPC scientific exploration and scientific machine learning (SciML). One challenging workload for CogSim is the replacement of one component in a complex physical simulation with a fast, learned, surrogate model that is "inside" of the computational loop. The execution of this in-the-loop inference is particularly challenging because it requires frequent inference across multiple possible target models, can be on the simulation's critical path (latency bound), is subject to requests from multiple MPI ranks, and typically contains a small number of samples per request. In this paper we explore the use of large, dedicated Deep Learning / AI accelerators that are disaggregated from compute nodes for this CogSim workload. We compare the trade-offs of using these accelerators versus the node-local GPU accelerators on leadership-class HPC systems.

==> 4_system_level_modeling.tex <==
\section{System-level Modeling}

Deep learning calculations have a natural appeal for being
able to be performed on a disaggregated system.  Neural networks
typically take a small number of inputs and have a small number of
outputs, but perform many computations.  In this section, we
build a modeling framework for exploring the feasibility of 
remote inference on a disaggregated accelerator using the Hermit
surrogate model to demonstrate our point.

\subsection{Neural Network Model}

Do we want to show how to model B/F ratios for neural nets?

\subsection{Moody Model}

Network capacity


